Nested bandits

In many online decision processes, the optimizing agent is called to choose between large numbers of alternatives with many inherent similarities; in turn, these similarities imply closely correlated losses that may confound standard discrete choice models and bandit algorithms. We study this question in the context of nested bandits, a class of adversarial multi-armed bandit problems where the learner seeks to minimize their regret in the presence of a large number of distinct alternatives with a hierarchy of embedded (non-combinatorial) similarities. In this setting, optimal algorithms based on the exponential weights blueprint (like Hedge, EXP3, and their variants) may incur significant regret because they tend to spend excessive amounts of time exploring irrelevant alternatives with similar, suboptimal costs. To account for this, we propose a nested exponential weights (NEW) algorithm that performs a layered exploration of the learner's set of alternatives based on a nested, step-by-step selection method. In so doing, we obtain a series of tight bounds for the learner's regret showing that online learning problems with a high degree of similarity between alternatives can be resolved efficiently, without a red bus / blue bus paradox occurring.

==> Conclusion.tex <==
%----------------------------------------------------------------------
%%% DISCUSSION
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


One limitation of the current framework is that the nested estimator \eqref{eq:NIWE-cost} requires knowledge of the intra-class cost increments $\incr_{\class}$ for every chosen similarity class $\class\ni\curr[\elem]$.
This is akin to the difference between the ``full bandit'' and ``semi-bandit'' setting that arises in combinatorial bandits \cite{CBL12}.
While relevant in a number of application domains (\eg in path-planning or when layering a structured security, such as the tranches of a CDO), treating the fully unobservable case \textendash\ possibly using an approach in the spirit of the hierarchical contextual analysis of \citet{SRYK+21} \textendash\ is an important open question for future research.

Finally, it is also interesting to note that our analysis has been carried out in an arbitrarily changing ``adversarial'' environment.
In a stochastic environment, it would be fruitful to consider other, contextual-based approaches such as LinUCB, KernelUCB and their variants \cite{LS20}.
Ideally, one would like to employ a nested variant of the ``universal'' algorithm of \citet{ZS19} that attains optimal regret guarantees in both stochastic and adversarial environments, but this question lies beyond the scope of our work.

==> Gentle.tex <==
%----------------------------------------------------------------------
%%% GENTLE
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


The nested logit choice has been first tackled by \citep{BA85}, introducing the Independence of Irrelevant Alternatives (IIA) property.
Namely, we would to have the logit model of sampling w.r.t. a score based estimate\TR{not sure I understand this sentence as is}, not to be sensitive to the artificial\TR{this is true even if the addition isn't artificial right?} add\TR{addition?} of irrelevant alternatives. For instance, if the action set is transportation ways\TR{consists in transportation modes} like car and bus, with say roughly same score estimates, you would potentially sample\TR{one would expect to sample} each alternative with $.5$ probability. The problem is if you add another bus, with same utility, but with different colors\TR{if another bus is added, with the same utility but a different color}. You end up having one blue bus, and one red bus in your set of choice. Then the usual logit model drops to $.33$ for each alternative, although you expect to sample the car as before, with $.5$ probability, based on the irrelevant alternatives (the bus you added)\TR{although you would ideally expect that the addition of the redundant alternative (the new bus) does not change the probability to sample the of the other alternative (the car)}. One way to circumvent this paradox is to model such a choice in a two-stage nested process. The action set is partitioned into embedded classes \MM{maybe removing all sets, and maths here would make more sense, only high level big picture exposing?} $\class\atlvl{1}^0, \class\atlvl{1}^1$, having several common characteristics\TR{which share common characteristics that translate in correlated/similar utilities}. The two-stage sampling process is based on first\TR{begins by first} choosing one of the two samples\TR{classes} $\class\atlvl{1}^0, \class\atlvl{1}^1$ with certain probability, depending of its previously estimated utility\TR{with probabilities depending of their respective estimated utility}, and then among this sampled class $\class\atlvl{1}^i$, the experimenter chooses alternative action\TR{and then continues by choosing $-$ among the sampled class $\class\atlvl{1}^i$ $-$ one of the corresponding actions} $\elem \in \class\atlvl{1}^i$, with some probability depending on the utility of such alternative\TR{with probabilities depending of their respective estimated utility}.
